American Stories: A Large-Scale Structured Text Dataset of Historical U.S. Newspapers

Existing full text datasets of U.S. public domain newspapers do not recognize the often complex layouts of newspaper scans, and as a result the digitized content scrambles texts from articles, headlines, captions, advertisements, and other layout regions. OCR quality can also be low. This study develops a novel, deep learning pipeline for extracting full article texts from newspaper images and applies it to the nearly 20 million scans in Library of Congress's public domain Chronicling America collection. The pipeline includes layout detection, legibility classification, custom OCR, and association of article texts spanning multiple bounding boxes. To achieve high scalability, it is built with efficient architectures designed for mobile phones. The resulting American Stories dataset provides high quality data that could be used for pre-training a large language model to achieve better understanding of historical English and historical world knowledge. The dataset could also be added to the external database of a retrieval-augmented language model to make historical information - ranging from interpretations of political events to minutiae about the lives of people's ancestors - more widely accessible. Furthermore, structured article texts facilitate using transformer-based methods for popular social science applications like topic classification, detection of reproduced content, and news story clustering. Finally, American Stories provides a massive silver quality dataset for innovating multimodal layout analysis models and other multimodal applications.

==> Figs/Pipeline.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=\linewidth]{Figs/pipeline.png}
    \caption{The four steps in the newspaper digitization pipeline.} 
    \label{fig:pipeline}
    \vspace{-2mm}
  \end{figure}

  

==> Figs/WireClusters.tex <==
\begin{figure}[ht]
    \centering
    \includegraphics[width=.6\linewidth]{Figs/Content-main.png}
    \caption{Wire articles. This figure represents....} 
    \label{fig:clusters}
    \vspace{-4mm}
  \end{figure}


==> Tables/legibility.tex <==
\begin{table}[t]
    \centering
    \resizebox{.5\linewidth}{!}{
    \begin{threeparttable}
       \begin{tabular}{lccc}
      \toprule
 & (1) & (2) & (3)   \\

Actual / Predicted	&	Legible	&	Borderline	&	Illegible	\\
  \cmidrule{2-4}
Legible	&	77	&	4	&	0	\\
Borderline	&	4	&	9	&	2	\\
Illegible	&	1	&	5	&	10	\\
      \bottomrule 
    \end{tabular}
    \end{threeparttable}
  }
    \caption{\textbf{Legibility Classification.}}
      \label{legibility_classification}
\end{table}

